BERT is not The Count: Learning to Match Mathematical Statements with Proofs

We introduce a task consisting in matching a proof to a given mathematical statement. The task fits well within current research on Mathematical Information Retrieval and, more generally, mathematical article analysis (Mathematical Sciences, 2014). We present a dataset for the task (the MATcH dataset) consisting of over 180k statement-proof pairs extracted from modern mathematical research articles. We find this dataset highly representative of our task, as it consists of relatively new findings useful to mathematicians. We propose a bilinear similarity model and two decoding methods to match statements to proofs effectively. While the first decoding method matches a proof to a statement without being aware of other statements or proofs, the second method treats the task as a global matching problem. Through a symbol replacement procedure, we analyze the "insights" that pre-trained language models have in such mathematical article analysis and show that while these models perform well on this task with the best performing mean reciprocal rank of 73.7, they follow a relatively shallow symbolic analysis and matching to achieve that performance.

==> Limitations.tex <==
\section{Limitations}
\label{sec:Limitations}

==> anon.tex <==
\section{Anonymization}

\subsection{Results}
\yftahcomment{I am writing here some points. I will transform them into a paragraph when I have the whole picture. Waylon, some of the points are taken directly from your observation section. If I misinterpreted them, please let me know.}
\begin{itemize}[noitemsep]
\item The adversarial anonymization results are almost as good as the zero anonymization results. The variables' shift in mathematical functionality did not harm the models' ability to match theorem and proof pairs. The slight performance drop indicates that the models rely on simple token matching instead of a deep understanding of the mathematical structure of the texts.
\item Customize vocabulary is crucial for performance. \yftahcomment{elaborate on some of the models} 
\item \yftahcomment{compare between global and local}
\item \yftahcomment{expand about the different anonymization methods}
\end{itemize}
\yftahcomment{Add tf-idf}

\noindent \wayloncomment{Anonymization details}

\wayloncomment{Common rules: 1. We only anonymize the variables that appear both in  the theorem and proof; 2. Consistency: if variable $a$ is mapped to $b$, all the lower case $a$ in the proof will be replaced by $b$s, the uppercase $A$ will be replced by $B$, bold $\bold{a}$ will be replaced by bold $\bold{b}$, script $\mathtt{a}$ will be replaced by script $\mathtt{b}$, etc.. However, we do not replace the double-struck letters like $\mathbb{R}$ since they usually represent mathematical fileds which contain specific semantic information; 3. Bijection: the anonymization mapping is a bijection and we try to avoid mapping a variable to itself unless there is no more available candidate; 4. Black list: to avoid the ambigution caused by some variables containing multiple English letters, we find all the variables that are longer than three English letters and use an English spellchecker PyEnchant to detect the English words. If a multiple-letter variable is detected as an English word, it will be added to the black list so that we can make sure we do not separate it.}

\wayloncomment{Partial: particularly for partial anonymization, we only replace 50\% of variables that appear both in the theorem and proof. The other variables will remain unchanged.}

\wayloncomment{Adversarial: nothing special I can think of for now}

\wayloncomment{Full: nothing special I can think of for now}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}








\subsection{Feature Importance Analysis}
To shed light on the terms that affect our models' predictions, we use LIME \cite{ribeiro2016should}, a prominent method for explainability via feature importance. We can use Lime to probe all of our models, as it is a model agnostic method. \yftahcomment{Should I provide some technical details about what Lime does?}
In Figure \yftahcomment{add figure} we can see how feature importance change over different anonymization levels. We observe \yftahcomment{add observations}


==> misc.tex <==
\paragraph{Baseline vs self-attentive systems}
We report baseline results in Table~\ref{tab:baselines}.
The best baseline is the TF-IDF model considering
both text and mathematical formulae as input,
it achieves an MRR of 29.9 and an accuracy of 23.8 (dev set).
These results suggest that the task is not trivial,
and that bag-of-words model are insufficiently
expressive to solve it.
In contrast, our best self-attentive model (Table~\ref{tab:conv-results}) 
%\marginpar{\textcolor{red}{Results not up to date for now}}
outperforms all baselines by a wide margin, 
obtaining an MRR of 64.5 and an accuracy of 57.8 (dev set, local decoding).
However, the neural model fails to improve over the baselines in the text-only setting, perhaps
due to the fact that the limitation in this setting is the lack of sufficient information,
which cannot be compensated by a higher model expressiveness.


\wayloncomment{MBERT and SBERT training: For the both types of BERT model, MathBERT and ScratchBERT, we fine-tune the pretrained MathBERT \cite{mathbert} and the ScratchBERT language model introduced in SBERT pretraining on the training set for 60 epochs with learning rate $l=2e-3$, an ASGD optimizer and an scheduler which scheduler multiplies learning rate by $0.99$ after each epoch. Due to the limitation of GPU memory, we can only set batch size $b=16$ for both local training and global training. We evaluate the model on the validation set every 5 epochs and select the one with highest validation accuracy.}

\wayloncomment{SBERT pretraining: For pretraining the SBERT language model, we first retrain a new wordpiece tokenizer with new vocabulary on our training set. Next we train the SBERT model on the masked language modeling (MLM) task on 4 GPUs using 8 as the batch size per device. We evaluate the language model every 500 steps where one step stands for training on one sentence and choose the one with best performance on the validation set.}

\wayloncomment{NPT training: For both local and global training, we perform 400 epochs over the whole training set on the self-attentive model. We use batches of size $b=60$ and set learning rate $l = 0.005$ of the ASGD optimizer based on preliminary experiments. An exponential learning rate scheduler (the learning rate is multiplied by $0.996$ after each epoch) is also used to stable the optimizer in latter training procedure (after 300 epochs). During training, we evaluate the model's performance on the validation set every 20 epochs and select the best one among these intermediate models. Particularly, we observed in initial experiments that training only with the global objective required a very long time and had a very slow convergence rate. Therefore, we used the following global-local objective: $\mathcal{L'}_{\textsc{loc}} + \mathcal{L}_{\textsc{glob}}$,
that we optimized by alternating one stochastic step for each loss.}

%Upon inspection of our global model incorrect predictions (`both' setting) on the development set, we found that a common source of error is due to the proof often introducing discourse-new concepts and new variables,
%while not necessarily repeating discourse-given concepts that occur in the statement.
%As a result, the set of variables and concepts in a proof might better match those of another statement. We provide examples of the model output in Appendix~A (supplementary material).
%Finally, incorrectly predicted proofs often contain highly polysemous words (\textit{linearly}, \textit{components}) that also occur in the statement.
%\yftahcomment{Shay, should we keep this?}\shaycomment{you could have such analysis, but it is not clear to me what you are saying, especially in the beginning paragraph.}


==> reviews_EACL.tex <==
Responses and action items for September ARR: 

Reviewer 5PLg [score - 3.5]:

We thank the reviewer for their comments.

> The paper lacks discussion about the concrete connections/differences between the proposed task and the MIR problem.

We agree. We will frame the problem of matching proofs to their corresponding statements as an essential sub-task of MIR. The basic premise is that such matching allows researchers to submit and process advanced queries to support their research.   

In the context of MIR, our task definition can be thought of as a proxy for a "proof generation" problem -- in which statements are proven based on a corpus of statements and proofs.


> In the proposed task, an assumption made is that the collection of statements and the collection of proofs are in the same size. Why is this necessary?

No, this assumption is not necessary. We mention it to make the exposition simpler. We can have a many-to-many matching using our algorithm. We will make it clearer in the paper.

Reviewer q1jH [score - 2.5]:

We thank the reviewer for their comments.

> My main concern and the main reason for my overall score is around the lack of clarity of the proposed symbol replacement methods and whether the resulting proofs are, in fact, valid from a mathematical perspective. [example given]

We elaborate more on the symbol replacement procedure in this context. We can use your example  - "a_0 = 5 a_1 = 6 forall i >= 2 : a_i = a_{i-1} + a_{i-2} Hence a_10". When we replace "a" for "x" *we do so consistently across all of "x" appearances* - "x_0 = 5 x_1 = 6 forall i >= 2 : x_i = x_{i-1} + x_{i-2} Hence a_10". Our symbol replacement is consistent and semantics-preserving.

More generally, we can pair each mathematical statement with the set of its symbols and then choose a subset to replace. Consider matrix multiplication "C = AxB, c_ij = sum_from_k=1_to_k=m(A_ik*B_kj)", the corresponding symbol list is - ["a", "b", "c", "i", "j", "k", "m"], for partial replacement, we randomly select 50\% of the symbols for replacement, for example - ["a", "c", "j", "k"], to be replaced (correspondingly) with this set - ["t", "q", "y", "x"] to get the following statement - "Q = TxB, q_iy = sum_from_x=1_to_x=m(T_ix*B_xy)". As you can see, each symbol was consistently replaced, where uppercase symbols follow lowercase and vice versa.

During the development of our symbol replacement procedure, we validated it with two graduate students who manually inspected over 100 theorem-proof pairs for each kind of symbol replacement. They found this process to be semantics-preserving in almost all cases.

We will include a more detailed account of this process and the exact way we do the symbol replacement.

> The connection to mathematical information retrieval (MIR) is not very clear.

We will frame the problem of matching proofs to their corresponding statements as an essential sub-task of MIR, allowing researchers to submit more advanced queries to support their research. 

> To the authors' credit, they acknowledge this disconnect and mitigate it using variable renaming. However, the mitigation isn't sufficient, in my opinion, as it doesn't change non-symbol aspects such as writing style.

We agree. We will elaborate on this limitation in the designated “Limitations” section. While our findings show that current models tend to rely heavily on mathematical inputs compared to textual ones (Table 5), we do plan to expand our research and include more realistic setups in the future. 

> The MATcH dataset, I presume, will be released upon publication. Please confirm!

Absolutely, we will make the dataset and the code publicly available upon acceptance. 

> I did not follow the reference (if any) in the first part of the title ("BERT is not the Count"). If you wish to keep it, please use some space to explain for the broader audience.

Since BERT is often referenced in NLP as the character from the children's show Sesame Street, we used another reference to this show -- the Count. More information about this character appears here: https://en.wikipedia.org/wiki/Count_von_Count ("... The Count's main role is to teach counting skills to children."). We will clarify this.

Reviewer gU86 [score - 2.5]:

We thank the reviewer for their comments.

> The contribution is incremental. Welleck et al.,2021 constructed NaturalProofs and proposed both the retrieval and generation tasks.

Our paper is quite different from Welleck's paper. Our paper presents the task of matching a proof to its corresponding theorem. Welleck et al.,2021 presented the task of reference retrieval (and generation), i.e., given a theorem, retrieve all the references that appear in its proof. For the generation variation, the references should be retrieved in an order-aware manner (corresponding to their order in the proof). While somewhat similar in their domain and relation to mathematics IR, our task is distinct from their two tasks, and generation is irrelevant to our case.

It is also noteworthy that the output of generation variation of reference retrieval is not a natural language but merely an ordered list of references. 

Finally, we introduce the notion of symbol replacement, which does not appear in Welleck et al.,2021.

> The local and global decoding methods are not novel, which are similar to the pairwise and joint parameterization in Welleck et al.,2021. However, I cannot find enough clarification for this.

As mentioned, the tasks are different. The type of model we have (a bilinear model to match two objects) has been used in many other contexts, including, for example, in word2vec.

In addition, the local/global distinction is different than the pairwise/joint distinction in the level of granularity of the models. Our global model finds a match for all statements (in the form of proofs). Welleck's joint parameterization finds all references for a *given* statement (so the model conditions on a single reference). These two things are entirely different in nature and goal. This means that the joint *model* of Welleck et al. is "local" and not global as our *decoding*. In addition, the joint model of Welleck et al. is still defined at the *instance* level, while our global decoding is defined at the *corpus* level.

> For a mathematical statement-proof dataset, the generation setting is more attractive for revealing how well the modern pre-trained language models can interpret/generate the proof with a given statement. I feel a bit regretful that the generation task is completely ignored in this paper.

We believe current methods are far from achieving good performance for such a challenging generation task and prefer to focus on the retrieval task as an intermediate (but still challenging) task. As mentioned before, Welleck et al.,2021 presented a  relaxation for the problem of reference generation (*not* proof generation, corresponding to our task), in which the desired output is an ordered list of references (which is not qualified as natural language). Even for such a more straightforward task relaxation, the results are far from promising (Table 8 in Welleck et al.'s paper).


Reviewer g46V [score - 3]:

We thank the reviewer for their comments.

> One challenge is scalabiliity and generalizability of their proposed global methods. Though inference time greedy algorithms provide some guarantees, their global assumptions alongwith comments about symbol replacement seems weak without experiments on established datasets such as NaturalProofs.

While we present results for a single dataset, we believe it to be highly comprehensive (over 180K theorem-proof pairs from multiple mathematical domains) and truly representative of our task (mathematical results taken from recently published academic papers).

In addition to being significantly larger than NaturalProofs (over seven times more data points), MATcH represents naturally-occurring statements and their proofs. More precisely, NaturalProofs consists of three different datasets: Proofwiki, the stacks project dump - which is a highly specialized math textbook, and Textbooks (a combination of " Introduction to Real Analysis" and "Elementary Number Theory: Primes, Congruences, and Secrets").

All of these resources are highly moderated, highly focused, simplified for the reader, and in most cases, serve undergrad math students, and deal with common theorems that do not require proof retrieval.

To conclude, we believe the MATcH dataset is larger, better-suited for our task, and more challenging and comprehensive than NaturalProofs.

> L91-92: A big question is how does the global method scale? Inference-time authors use LAP-MOD type sparse strategies, but even in this dataset, their global loss does not converge. It is also not "surprising" that a global strategy works better than a greedy one. I am not fully certain of the insight to gain from this.

The global model scales well, as we do not have to apply it to the full dataset but rather to a batch that can be as large as we wish. As an auxiliary objective, the global model improves the results, which is one reason to use it. Using a global model is indeed expected to outperform a local model, as has been documented in the literature. The critical thing is to balance the trade-off between computational efficiency and performance.

> L278: Is this true? Again, for the sake scalability; especially short proofs can definitely be assigned to many theorems. But, you remove them. Is this why?”

[[Line 278 says - “: a proof can be assigned only to a single statement.”]]

During our early experimentation with the dataset, we noticed local decoding results in an "unfair" assignment, i.e., some proofs are assigned to more than one statement and some to none (for full details, see Table 6). While it could be the case that for some proofs, one can find more than one matching statement, integrating our assumption into the model yields improvements across all the models, thus, strengthening our initial confidence in it. We will make it clear in the paper.

